GraphDCA -- a Framework for Node Distribution Comparison in Real and Synthetic Graphs

We argue that when comparing two graphs, the distribution of node structural features is more informative than global graph statistics which are often used in practice, especially to evaluate graph generative models. Thus, we present GraphDCA - a framework for evaluating similarity between graphs based on the alignment of their respective node representation sets. The sets are compared using a recently proposed method for comparing representation spaces, called Delaunay Component Analysis (DCA), which we extend to graph data. To evaluate our framework, we generate a benchmark dataset of graphs exhibiting different structural patterns and show, using three node structure feature extractors, that GraphDCA recognizes graphs with both similar and dissimilar local structure. We then apply our framework to evaluate three publicly available real-world graph datasets and demonstrate, using gradual edge perturbations, that GraphDCA satisfyingly captures gradually decreasing similarity, unlike global statistics. Finally, we use GraphDCA to evaluate two state-of-the-art graph generative models, NetGAN and CELL, and conclude that further improvements are needed for these models to adequately reproduce local structural features.

==> archived/feature_extractors.tex <==
\section{Structural similarity feature extractors}

{\color{blue} Motivation + problem setup + hint on 2 components of the framework (fe, scores) + verification benchmark, subsection on feature extractors, subsection on score, subsection about the dataset}

The GraphDCA similarity evaluation framework, described in Section \ref{sec:framework}, compares two graphs by viewing them as two sets of node features.
The framework is generic with respect to the choice of features under a single condition: that the feature spaces are consistent when extracted for different graphs.
% features reflect the same properties when extracted for different graphs. {\color{blue} < - PP : I don't get this}
This means that adjacency capturing features which are learned per graph \cite{perozzi_deepwalk_2014, grover_node2vec_2016, qiu_network_2018} cannot be used in our framework without modification.
There currently exists many different node representation learning approaches which adheres to this condition, and it is up to the practitioner to choose the feature extractor which best captures the properties relevant to their data and task.

In domains where nodes have additional attributes, e.g.\ chemical properties in molecular graphs \cite{szklarczyk2019string, gene2019gene}, product descriptors in co-purchase networks \cite{Bhatia16} or paper descriptors in citation graphs \cite{wang2020microsoft}, graph neural networks, such as the models by \cite{KipfW17, graphsage_hamilton17, velickovic2018graph, chiang2019cluster, graphsaint-iclr20}, may produce appropriate representations such that nodes with similar attributes are likely to have similar representations. 

In contrast, we are interested in node representations which capture \emph{structural} similarity.
Thus, we consider feature extractors that encode local connectivity structure around nodes, do not take into account node proximity in the graph, do not assume that any additional attributes are given and that do not rely on supervised pretraining using node labels which may be expensive to acquire for a generic graph.
There exists many feature extractors in this category \cite{henderson_its_2011, henderson_rolx_2012, ribeiro2017struc2vec, donnat_learning_2018, qiu_gcc_2020} out of which we have selected two of the latest works and a set of manually defined features.


{\bf Manual features}
A straight-forward approach for constructing node structural representations explicitly is to compute features from each node's $\rho$-egonet defined as the induced subgraph of all nodes within shortest path distance $\rho$ as previously done for $\rho=1$ \cite{everett1990ego, akoglu_oddball_2010}.
However, selecting a single radius $\rho$ may be difficult as different radii likely expose different local structures.
To circumvent this issue, we compute and concatenate features for all $\rho \leq 4$. 
Specifically, we calculate the following commonly used graph statistics of the egonets as features: number of nodes, average and max node degree, number of triangles, global clustering coefficient \cite{newman2003structure} and assortativity coefficient \cite{newman2003mixing}.


%\subsubsection{GraphWave}
{\bf GraphWave} \cite{donnat_learning_2018} produces structural embeddings for each node by considering the diffusion of a spectral graph wavelet centered at a node. 
Features are constructed from these wavelets by treating them as probability distributions on the graph and characterizing the distributions using the corresponding empirical characteristic functions. 
GraphWave is a deterministic method that scales linearly with the number of edges in the graph.

%\subsubsection{GCC}
{\bf Graph Contrastive Coding (GCC)} \cite{qiu_gcc_2020} uses contrastive learning to learn structural representations of nodes. Data instances representing a node are formed by constructing subgraphs using random walk based graph sampling initialized at the node. A graph neural network is used to encode these subgraphs into latent representations. The contrastive loss is defined such that a low loss is achieved when instances originating from the same node have similar latent representations while a high loss is obtained for representations of instances originating from different nodes. Similarly to successful models for natural language processing and computer vision, GCC is meant to be pre-trained on a diverse set of graphs and the pre-trained model can then be used for downstream tasks on other graphs. 



==> archived/method.tex <==
\section{Graph similarity evaluation framework}
\label{sec:framework}




%\subsection{Graph comparison based on feature extractors (we can give it a name later)}
To address the challenges outlined above, we propose a different approach. Instead of comparing graphs directly, we propose to compare their \emph{properties} defined by a feature extractor of choice. The goal is to build a framework that:
\begin{itemize}
    \item captures local structural features of graphs
    \item does not require manual feature engineering
    \item is able to prioritize specific node types
\end{itemize}


Given an input graph $G = (V, E)$ with a vertex set $V$ and an edge set $E$, and a feature extractor $f_G: V \to  \mathbb{R}^d$, we define similarity on graphs in terms of similarity of their features $f(G) = \{r_1, \dots, r_N\}$ where $f_G(v_i) = r_i$.

Our goal is to construct a framework where similarity between two graphs $G_1$ and $G_2$ is expressed through $f(G_1)$ and $f(G_2)$.
%{\color{blue} Expectations of the framework: Node permutation invariance, local feature extractors, motivation for DCA - similar nodes are close, no need for downstream task, able to focus on specific nodes}



%\newline
{\bf Delaunay Component Analysis (DCA)} is a framework for comparing two sets of embeddings, $R_1, R_2 \subset \mathbb{R}^d$, where $d$ is the dimensionality of the embedding space. The idea of DCA is to compare the sets by analyzing the connected components of the manifold represented by $R_1 \cup R_2$. Intuitively, if $R_1$ and $R_2$ contribute to each connected component equally and homogeneously they are considered similar. The manifold $R_1 \cup R_2$ is approximated by a so-called ``distilled'' Delaunay graph. First, a Delaunay graph $\mathcal{D}$ is built to efficiently capture the neighborhood structure of the representation space. Since $\mathcal{D}$ is always connected by construction, a modified version of the HDBSCAN \cite{McInnes2017} clustering algorithm is then applied to the minimum spanning tree of $\mathcal{D}$ to group the points into clusters $\{\mathcal{D}_c\}$ representing the connected components. This procedure requires tuning the minimum clustering size (mcs) hyperparameter inherent to HDBSCAN that defines the minimum number of points defining a cluster. The obtained connected components $\{\mathcal{D}_c\}$ are then analyzed in terms of $R_1$ and $R_2$ points and edges among them as summarized below.  

{\bf Similarity scores.} {\color{blue} Redefine the notation} DCA defines several scores to evaluate the alignment of $R_1$ and $R_2$. We consider three of them: \textit{network quality} which summarizes the total geometric alignment of $R_1$ and $R_2$ across all $\mathcal{D}_c$, and \textit{precision and recall} which reflect the ratio of $R_2$ and $R_1$, respectively, contained in geometrically rich components. Since we are interested in analyzing the node structural features, we modify the DCA framework such that we are able to calculate the scores only using specific nodes. {\color{blue} Add some motivation for this.} We therefore adjust the definitions of the scores given by~\cite{anonymous2022delaunay} as explained below. %To distinguish input graphs $G_k, k = 1, 2$ from the Delaunay graph $\mathcal{D}$ built on the representations $f(G_k)$, we use calligraphic notation $\mathcal{H}$ when referring to any subgraph $\mathcal{H}$ extracted from $\mathcal{D}$.

\textbf{Notation} Let $\mathcal{H} = (\mathcal{V}, \mathcal{E})$ be a \emph{latent} graph built on representations $f(G) = \{r_i\}_i$ of a given \emph{input} graph $G = (V, E)$. Let $\{w_j\}$ be a set of weights defined on the nodes $v_j \in V$ of $G$, which are further inherited to the representations $r_j$. 
Let $|\mathcal{H}|_{\mathcal{E}}$ denote the cardinality of the edge set of the latent graph $\mathcal{H}$, and let $\mathcal{H}^{R} = (\mathcal{V}|_R, \mathcal{E}_{R \times R})$ be the restriction of $\mathcal{H}$ to a set $R$. Furthermore, let $w(\mathcal{H}) = \sum_{r_j \in \mathcal{V}} w_j$ be the sum of weights of nodes (representations) of a graph $\mathcal{H}$. 

The considered DCA scores are aggregated local scores assessing the quality of each connected component. A Delaunay connected component $\mathcal{D}_c$ is said to be of high quality if points from $R_1$ and $R_2$ are geometrically well aligned.  This is achieved when the number of edges connecting representations from $R_1$ and $R_2$ is large compared to the number of edges in the restrictions $\mathcal{D}_c^{R_1}$ and $\mathcal{D}_c^{R_2}$ of $\mathcal{D}_c$ to $R_1$ and $R_2$.  

\begin{definition}
The quality $q \in [0, 1]$ of a connected component $\mathcal{D}_c$ of a Delaunay graph $\mathcal{D}$ is defined as 
\begin{align*}
    q(\mathcal{D}_c) = \begin{cases}
    1 -  \frac{(|\mathcal{D}_i^{R_1}|_\mathcal{E} + |\mathcal{D}_i^{E}|_\mathcal{E})}{|\mathcal{D}_i|_\mathcal{E}} & \text{if } |\mathcal{D}_i|_\mathcal{E} \geq 1,\\
    0              & \text{otherwise.}
    \end{cases}
\end{align*}
We define $\mathcal{D}_c$ as a \textit{fundamental} component if $q(\mathcal{D}_c) > 0$ and denote by $\mathcal{F}$ the union of all fundamental components of $\mathcal{D}$. Moreover, the quality of the entire Delaunay graph $q(\mathcal{D})$ is called network quality.
\end{definition}

However, network quality itself does not provide insights into the position of the node features, for example, how many nodes are contained in fundamental components which is measured by precision and recall scores. However, in order to be able to focus such analysis on specific nodes, we adjust the original definitions to a scenario where nodes can be given weights. Note that by using uniform weights, we recovered the definitions given by~\cite{anonymous2022delaunay}.

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \input{figures/graphs/star}
    \caption{Star}
    \label{fig:star}
\end{subfigure}
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \input{figures/graphs/wheel}
    \caption{Wheel}
    \label{fig:wheel}
\end{subfigure}
\\
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \input{figures/graphs/diamond}
    \caption{Diamond}
    \label{fig:diamond}
\end{subfigure}
\begin{subfigure}[b]{0.2\textwidth}
    \centering
    \input{figures/graphs/friendship}
    \caption{Friendship}
    \label{fig:friendship}
\end{subfigure}
\caption{Subgraphs used for synthetic dataset}
\label{fig:subgraphs}
\end{figure}
 
\begin{definition}
We define the weighted precision $p_w \in [0, 1]$ and weighted recall $r_w \in [0, 1]$ of $\mathcal{D}$ as 
\begin{align*}
   p_w = \frac{\sum_{\mathcal{D}_c \in \mathcal{F}}w(\mathcal{D}_c^{R_2})}{w(\mathcal{D}^{R_2})} \quad \text{and} \quad r_w = \frac{\sum_{\mathcal{D}_c \in \mathcal{F}}w(\mathcal{D}_c^{R_1})}{w(\mathcal{D}^{R_1})}.
\end{align*}
\end{definition}

Since all the scores are normalized and it holds that the higher the better, we report a unified score defined as their harmonic mean:
\begin{definition}
We define the weighted DCA score $s_{\wDCA}$ among feature sets $R_1$ and $R_2$ corresponding to the input graphs $G_1$ and $G_2$ as 
\begin{align}
   s_{\wDCA}(R_1, R_2) = h (p_w, r_w, q)  \label{eq:dca_similarity}
\end{align}
where $h$ is the harmonic mean. 
\end{definition}




\subsection{Synthetic dataset}
\label{sec:synthetic-dataset}
In addition to the GraphDCA framework, we contribute with a synthetic dataset of undirected graphs having different local structures. 

Each synthetic graph consists of a main graph into which smaller subgraphs of a specific type are inserted. We are considering two types of main graphs: cycle and tree. The tree graph is constructed by attaching each new node to the graph by adding a single edge between the new node and a node sampled uniformly from the nodes already in the graph.  

For the subgraphs, we are considering the following five types: star, wheel, diamond, friendship and random. The first four are deterministic given a degree of the central node and the total number of nodes, visualized in Figure \ref{fig:subgraphs} for central degree of four and $20$ total nodes with the central nodes marked in blue.
These are all generalizations of the graphs that are typically called star, wheel, diamond and friendship in graph theory.

The random subgraphs are created by first connecting the central node with new nodes until it has the desired degree and then a chosen number of edges are sampled uniformly between all nodes except the central node. Finally, to make sure the random subgraph is connected, each connected component is connected to the component containing the central node with a random edge, excluding edges to the central node.

To insert the subgraphs into the main graph, each subgraph is connected to the main graph by a predetermined number of edges between randomly chosen nodes in the subgraph and randomly chosen nodes in the main graph. 

All of our graphs are generated using a main graph with $1000$ nodes and $20$ instances of subgraphs comprised of $40$ nodes and central degree of four. For the random subgraphs $46$ random edges are sampled before all components are connected. Each subgraph is connected to the main graph with four edges. In total, each $G$ contains $1800$ nodes. %Each subgraph is connected to the main graph with four edges. 
We use superscript to denote the type of the main graph and subscript for the type of the subgraphs inserted, e.g., $G_s^m = G^{\text{tree}}_{\text{diamond}}$ denotes a graph with $m = \textit{tree}$ main graph and $s = \textit{diamond}$ subgraphs. We omit the explicit notation of the main graph type when no confusion can arise.





%Each synthetic graph consists of a main graph which is connected with subgraphs of one or several types. The chosen subgraphs all have a central node with the same degree. We are considering the following five types of subgraphs: diamond, friendship, sampled edges, star and wheel.  Each subgraph is then connected to the main graph by a predetermined number of edges with each edge connecting a ramdomly chosen node in the subgraph to a randomly chosen node in the main graph. 

%All of our graphs are generated using a main graph with $1000$ nodes and $20$ instances of subgraphs with $40$ nodes each. Each subgraph is connected to the main graph with four edges. 






==> figures/temp_tex/change_main_graph_f1_h_marked_weights_mcs2.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.105882352941176,0.619607843137255,0.466666666666667}
\definecolor{color1}{rgb}{0.850980392156863,0.372549019607843,0.00784313725490196}
\definecolor{color2}{rgb}{0.458823529411765,0.43921568627451,0.701960784313725}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=none},
tick align=outside,
tick pos=left,
title={egonet},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\path [draw=color0, line width=1pt]
(axis cs:0,0.913)
--(axis cs:0,0.979);

\path [draw=color0, line width=1pt]
(axis cs:1,0.532)
--(axis cs:1,0.734);

\path [draw=color0, line width=1pt]
(axis cs:2,0.366)
--(axis cs:2,0.562);

\path [draw=color0, line width=1pt]
(axis cs:3,0.858)
--(axis cs:3,0.902);

\path [draw=color0, line width=1pt]
(axis cs:4,0.941)
--(axis cs:4,0.963);

\path [draw=color0, line width=1pt]
(axis cs:0,0.41)
--(axis cs:0,0.594);

\path [draw=color0, line width=1pt]
(axis cs:1,0.423)
--(axis cs:1,0.507);

\path [draw=color0, line width=1pt]
(axis cs:2,0.36)
--(axis cs:2,0.426);

\path [draw=color0, line width=1pt]
(axis cs:3,0.53)
--(axis cs:3,0.6);

\path [draw=color0, line width=1pt]
(axis cs:4,0.583)
--(axis cs:4,0.753);

\addplot [line width=1pt, color0, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0 0.946
1 0.633
2 0.464
3 0.88
4 0.952
};
\addlegendentry{different}
\addplot [line width=1pt, color0, dashed, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0 0.502
1 0.465
2 0.393
3 0.565
4 0.668
};
\addlegendentry{different}

\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=none},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={gcc},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
yticklabels={}
]
\path [draw=color1, line width=1pt]
(axis cs:0,0.676)
--(axis cs:0,0.77);

\path [draw=color1, line width=1pt]
(axis cs:1,0.554)
--(axis cs:1,0.718);

\path [draw=color1, line width=1pt]
(axis cs:2,0.423)
--(axis cs:2,0.699);

\path [draw=color1, line width=1pt]
(axis cs:3,0.607)
--(axis cs:3,0.889);

\path [draw=color1, line width=1pt]
(axis cs:4,0.651)
--(axis cs:4,0.801);

\path [draw=color1, line width=1pt]
(axis cs:0,0.612)
--(axis cs:0,0.702);

\path [draw=color1, line width=1pt]
(axis cs:1,0.481)
--(axis cs:1,0.611);

\path [draw=color1, line width=1pt]
(axis cs:2,0.434)
--(axis cs:2,0.55);

\path [draw=color1, line width=1pt]
(axis cs:3,0.4)
--(axis cs:3,0.804);

\path [draw=color1, line width=1pt]
(axis cs:4,0.514)
--(axis cs:4,0.686);

\addplot [line width=1pt, color1, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 0.723
1 0.636
2 0.561
3 0.748
4 0.726
};
\addlegendentry{different}
\addplot [line width=1pt, color1, dashed, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 0.657
1 0.546
2 0.492
3 0.602
4 0.6
};
\addlegendentry{different}

\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=none},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={graphwave},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
yticklabels={}
]
\path [draw=color2, line width=1pt]
(axis cs:0,0.67)
--(axis cs:0,0.782);

\path [draw=color2, line width=1pt]
(axis cs:1,0.536)
--(axis cs:1,0.854);

\path [draw=color2, line width=1pt]
(axis cs:2,0.494)
--(axis cs:2,0.6);

\path [draw=color2, line width=1pt]
(axis cs:3,0.613)
--(axis cs:3,0.833);

\path [draw=color2, line width=1pt]
(axis cs:4,0.707)
--(axis cs:4,0.801);

\path [draw=color2, line width=1pt]
(axis cs:0,0.351)
--(axis cs:0,0.509);

\path [draw=color2, line width=1pt]
(axis cs:1,0.503)
--(axis cs:1,0.577);

\path [draw=color2, line width=1pt]
(axis cs:2,0.472)
--(axis cs:2,0.502);

\path [draw=color2, line width=1pt]
(axis cs:3,0.458)
--(axis cs:3,0.554);

\path [draw=color2, line width=1pt]
(axis cs:4,0.347)
--(axis cs:4,0.585);

\addplot [line width=1pt, color2, mark=square*, mark size=3, mark options={solid}]
table {%
0 0.726
1 0.695
2 0.547
3 0.723
4 0.754
};
\addlegendentry{different}
\addplot [line width=1pt, color2, dashed, mark=square*, mark size=3, mark options={solid}]
table {%
0 0.43
1 0.54
2 0.487
3 0.506
4 0.466
};
\addlegendentry{different}
\end{groupplot}

\end{tikzpicture}


==> figures/temp_tex/test.tex <==
% This file was created by tikzplotlib v0.9.2.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.105882352941176,0.619607843137255,0.466666666666667}
\definecolor{color1}{rgb}{0.850980392156863,0.372549019607843,0.00784313725490196}
\definecolor{color2}{rgb}{0.458823529411765,0.43921568627451,0.701960784313725}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=none},
tick align=outside,
tick pos=left,
title={egonet},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
ytick={0,0.2,0.4,0.6,0.8,1},
yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\path [draw=color0, line width=1pt]
(axis cs:0,0.913)
--(axis cs:0,0.979);

\path [draw=color0, line width=1pt]
(axis cs:1,0.532)
--(axis cs:1,0.734);

\path [draw=color0, line width=1pt]
(axis cs:2,0.366)
--(axis cs:2,0.562);

\path [draw=color0, line width=1pt]
(axis cs:3,0.858)
--(axis cs:3,0.902);

\path [draw=color0, line width=1pt]
(axis cs:4,0.941)
--(axis cs:4,0.963);

\path [draw=color0, line width=1pt]
(axis cs:0,0.41)
--(axis cs:0,0.594);

\path [draw=color0, line width=1pt]
(axis cs:1,0.423)
--(axis cs:1,0.507);

\path [draw=color0, line width=1pt]
(axis cs:2,0.36)
--(axis cs:2,0.426);

\path [draw=color0, line width=1pt]
(axis cs:3,0.53)
--(axis cs:3,0.6);

\path [draw=color0, line width=1pt]
(axis cs:4,0.583)
--(axis cs:4,0.753);

\addplot [line width=1pt, color0, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0 0.946
1 0.633
2 0.464
3 0.88
4 0.952
};
\addlegendentry{different}
\addplot [line width=1pt, color0, dashed, mark=triangle*, mark size=3, mark options={solid,rotate=180}]
table {%
0 0.502
1 0.465
2 0.393
3 0.565
4 0.668
};
\addlegendentry{different}

\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=none},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={gcc},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
yticklabels={}
]
\path [draw=color1, line width=1pt]
(axis cs:0,0.676)
--(axis cs:0,0.77);

\path [draw=color1, line width=1pt]
(axis cs:1,0.554)
--(axis cs:1,0.718);

\path [draw=color1, line width=1pt]
(axis cs:2,0.423)
--(axis cs:2,0.699);

\path [draw=color1, line width=1pt]
(axis cs:3,0.607)
--(axis cs:3,0.889);

\path [draw=color1, line width=1pt]
(axis cs:4,0.651)
--(axis cs:4,0.801);

\path [draw=color1, line width=1pt]
(axis cs:0,0.612)
--(axis cs:0,0.702);

\path [draw=color1, line width=1pt]
(axis cs:1,0.481)
--(axis cs:1,0.611);

\path [draw=color1, line width=1pt]
(axis cs:2,0.434)
--(axis cs:2,0.55);

\path [draw=color1, line width=1pt]
(axis cs:3,0.4)
--(axis cs:3,0.804);

\path [draw=color1, line width=1pt]
(axis cs:4,0.514)
--(axis cs:4,0.686);

\addplot [line width=1pt, color1, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 0.723
1 0.636
2 0.561
3 0.748
4 0.726
};
\addlegendentry{different}
\addplot [line width=1pt, color1, dashed, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 0.657
1 0.546
2 0.492
3 0.602
4 0.6
};
\addlegendentry{different}

\nextgroupplot[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=none},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
tick pos=left,
title={graphwave},
x grid style={white!80!black},
xmajorgrids,
xmin=-0.2, xmax=4.2,
xtick style={color=white!15!black},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xtick={0,1,2,3,4},
xticklabel style = {rotate=30.0},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
xticklabels={diamond,friendship,samplededges,star,wheel},
y grid style={white!80!black},
ylabel={Similarity score},
ymajorgrids,
ymin=0, ymax=1,
ytick style={color=white!15!black},
yticklabels={}
]
\path [draw=color2, line width=1pt]
(axis cs:0,0.67)
--(axis cs:0,0.782);

\path [draw=color2, line width=1pt]
(axis cs:1,0.536)
--(axis cs:1,0.854);

\path [draw=color2, line width=1pt]
(axis cs:2,0.494)
--(axis cs:2,0.6);

\path [draw=color2, line width=1pt]
(axis cs:3,0.613)
--(axis cs:3,0.833);

\path [draw=color2, line width=1pt]
(axis cs:4,0.707)
--(axis cs:4,0.801);

\path [draw=color2, line width=1pt]
(axis cs:0,0.351)
--(axis cs:0,0.509);

\path [draw=color2, line width=1pt]
(axis cs:1,0.503)
--(axis cs:1,0.577);

\path [draw=color2, line width=1pt]
(axis cs:2,0.472)
--(axis cs:2,0.502);

\path [draw=color2, line width=1pt]
(axis cs:3,0.458)
--(axis cs:3,0.554);

\path [draw=color2, line width=1pt]
(axis cs:4,0.347)
--(axis cs:4,0.585);

\addplot [line width=1pt, color2, mark=square*, mark size=3, mark options={solid}]
table {%
0 0.726
1 0.695
2 0.547
3 0.723
4 0.754
};
\addlegendentry{different}
\addplot [line width=1pt, color2, dashed, mark=square*, mark size=3, mark options={solid}]
table {%
0 0.43
1 0.54
2 0.487
3 0.506
4 0.466
};
\addlegendentry{different}
\end{groupplot}

\end{tikzpicture}
